Optimal Feed-Forward Control for Robotic Transportation of Solid and Liquid Materials via Nonprehensile Grasp

In everyday life, we often find that we can maintain an object's equilibrium on a tray by adjusting its orientation. Building upon this observation and extending the method we previously proposed to suppress sloshing in a moving vessel, this paper presents a feedforward control approach for transporting objects with a robot that are not firmly grasped but simply placed on a tray. The proposed approach combines smoothing actions and end-effector re-orientation to prevent object sliding. It can be integrated into existing robotic systems as a plug-in element between the reference trajectory generator and the robot control. To demonstrate the effectiveness of the proposed methods, particularly when dealing with unknown reference signals, we embed them in a direct teleoperation scheme. In this scheme, the user commands the robot carrying the tray by simply moving their hand in free space, with the hand's 3D position detected by a motion capture system. Furthermore, in the case of point-to-point motions, the same feedforward control, when fed with step inputs representing the desired goal position, dynamically generates the minimum-time reference trajectory that complies with velocity and acceleration constraints, thus avoiding sloshing and slipping. More information and accompanying videos can be found at https://sites.google.com/view/robotwaiter/

==> trjfilter2.tex <==
%\def\dy{\dot y}
%\def\ddy{\ddot y}
%\def\um{\dddot x_{\mbox{\tiny{m}}}}
%\def\uM{\dddot x_{\mbox{\tiny{M}}}}
%\def\dym{\dot y_{\mbox{\tiny{m}}}}
%\def\dyM{\dot y_{\mbox{\tiny{M}}}}
%\def\ddym{\ddot y_{\mbox{\tiny{m}}}}
%\def\ddyM{\ddot y_{\mbox{\tiny{M}}}}
%\def\umM{(\um-\uM)}
%%\def\umM{\ddot x_{\mbox{\tiny{mM}}}}
%\def\D{(\ddy^2 - 2\dy\uM)}

\def\dy{\dot y}
\def\ddy{\ddot y}
%\def\dddxm{\jerk_{\mbox{\tiny{m}}}}
%\def\um{\dddxm}
%\def\dddxM{\jerk_{\mbox{\tiny{M}}}}
%\def\uM{\dddxM}
%\def\ddxm{\acc_{\mbox{\tiny{m}}}}
%\def\ddxM{\acc_{\mbox{\tiny{M}}}}
%\def\dxm{\vel_{\mbox{\tiny{m}}}}
%\def\dxM{\vel_{\mbox{\tiny{M}}}}
%\def\dym{\dot y_{\mbox{\tiny{m}}}}
%\def\dyM{\dot y_{\mbox{\tiny{M}}}}
%\def\ddym{\ddot y_{\mbox{\tiny{m}}}}
%\def\ddyM{\ddot y_{\mbox{\tiny{M}}}}


\newcommand{\xM}[1]{\overline{x}_{#1}}
\newcommand{\xm}[1]{\underline{x}_{#1}}

\newcommand{\yM}[1]{\overline{y}_{#1}}
\newcommand{\ym}[1]{\underline{y}_{#1}}

\def\dddxm{\xm{0}}
\def\um{\dddxm}
\def\dddxM{\xM{0}}
\def\uM{\dddxM}
\def\ddxm{\xm{1}}
\def\ddxM{\xM{1}}
\def\dxm{\xm{2}}
\def\dxM{\xM{2}}
\def\dym{\ym{2}}
\def\dyM{\yM{2}}
\def\ddym{\ym{1}}
\def\ddyM{\yM{1}}

\def\umM{(\um-\uM)}
%\def\umM{\ddot x_{\mbox{\tiny{mM}}}}
\def\Dp{(y_1^2 - 2y_2\um)}
\def\Dm{(y_1^2 - 2y_2\uM)}

\def\uu{\hat u_1}
\def\ud{\hat u_2}
\def\udu{(\ud-\uu)}
\def\uud{(\uu-\ud)}

\def\Dd{(y_1^2 - 2y_2\ud)}
\def\Du{(y_1^2 - 2y_2\uu)}


